Hiding speaker's sex in speech using zero-evidence speaker representation in an analysis/synthesis pipeline

The use of modern vocoders in an analysis/synthesis pipeline allows us to investigate high-quality voice conversion that can be used for privacy purposes. Here, we propose to transform the speaker embedding and the pitch in order to hide the sex of the speaker. ECAPA-TDNN-based speaker representation fed into a HiFiGAN vocoder is protected using a neural-discriminant analysis approach, which is consistent with the zero-evidence concept of privacy. This approach significantly reduces the information in speech related to the speaker's sex while preserving speech content and some consistency in the resulting protected voices.

==> figures/mos_box_plot.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
width=0.4\textwidth,
height=4cm,
xmin=-0.25, xmax=2.25,
xtick={0,0.5,1,1.5,2},
xticklabels={original,np,p,global,tdpsola},
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=5,
ytick style={color=black},
ytick={0,1,2,3,4,5}
]


%%ORIGINAL

\addplot [black]
table {%
-0.075 4.103233
0.075 4.103233
0.075 4.5748353
-0.075 4.5748353
-0.075 4.103233
};
\addplot [black]
table {%
0 4.103233
0 3.3994603
};
\addplot [black]
table {%
0 4.5748353
0 5.036936
};
\addplot [black]
table {%
-0.0375 3.3994603
0.0375 3.3994603
};
\addplot [black]
table {%
-0.0375 5.036936
0.0375 5.036936
};
\addplot [black, mark=o, mark size=0.3, mark options={solid,fill opacity=0}, only marks]
table {%
0 3.2099605
0 3.0927086
0 3.2917829
0 2.9618113
0 2.2294466
0 2.0910113
0 3.3648005
0 2.5094693
0 3.0803561
0 3.0983958
0 3.3172889
0 1.9086933
0 2.6188693
0 2.0194142
0 2.975424
0 2.5995243
0 2.5607648
0 2.5174117
0 2.4487972
0 3.1557243
0 2.3660893
0 3.2280881
0 2.6610794
0 3.1487017
0 3.3319376
0 2.9785097
0 3.0246358
0 2.6687064
0 2.6686263
0 2.94584
0 2.329637
0 2.586257
0 2.4670417
0 3.3774507
0 2.691932
0 3.0079594
0 2.2042975
0 2.5619366
0 2.5468729
0 2.7007759
0 3.083687
0 1.9527822
0 2.579958
0 3.2604806
0 3.1362221
0 3.33549
0 2.6625464
0 2.9623861
0 2.35464
0 2.6677337
0 3.096146
0 2.696642
0 1.8238369
0 2.7510445
0 3.3200269
0 3.0567787
0 3.1574426
0 3.2297444
0 2.2863286
0 3.321395
0 3.088078
0 2.7035747
0 3.1333604
0 3.0019763
0 3.3684785
0 2.3754845
0 3.3922944
0 2.8776479
0 2.9759781
0 2.5384233
0 2.4452822
0 2.615576
0 3.3054528
0 2.973498
0 2.6426208
0 3.2790813
0 3.3893192
0 3.1775205
0 2.2891645
0 3.1682394
0 3.0627756
0 2.9422398
0 3.2264016
0 2.965747
0 2.6355858
0 3.3625038
0 3.2995884
0 1.8492818
0 1.7420262
0 2.927557
0 3.046276
0 2.391263
0 3.1631384
0 2.72962
0 2.8632934
0 3.379962
0 2.979155
0 2.259083
0 3.0482914
0 2.4390683
0 3.0246336
0 3.025006
0 2.5945058
0 2.867046
0 3.174789
0 2.6552668
0 3.3867254
0 3.0739276
0 1.7123573
0 2.173694
0 1.8481746
0 2.7508824
0 3.3626137
0 2.17441
0 2.9947708
0 2.3461666
0 3.1398203
0 2.7567742
0 2.8863587
0 2.787306
0 3.0460668
0 2.6156456
0 2.8717434
0 2.6758137
0 2.778843
0 3.3566508
0 3.15354
0 3.276519
0 2.501688
0 3.102736
0 3.1905975
0 3.196873
0 3.052915
0 3.2180738
0 2.991717
0 3.138886
0 3.3784957
0 2.6360166
0 2.2114632
0 2.8058538
0 3.213049
0 2.98953
0 2.6014993
0 3.3327022
0 2.263169
0 2.8652284
0 3.3732734
0 2.2804236
0 2.546551
0 2.2150998
0 3.1933079
0 2.4976315
0 3.3560143
0 2.989038
0 2.004202
0 3.36825
0 3.1338341
0 3.1986794
0 1.9975638
0 1.8140101
0 3.0906324
0 3.1372757
0 3.1269374
0 2.223224
0 2.8515353
0 2.4346514
0 2.1590352
0 3.3801582
0 2.930549
0 2.99676
0 2.906059
0 3.2909474
0 3.301505
0 3.0289724
0 2.9624372
0 3.210363
0 3.1347866
0 3.3080964
0 2.7563746
0 3.3042307
0 2.7971895
0 2.0291767
0 3.379735
0 2.2238233
0 3.1702971
0 3.3441324
0 3.3352952
0 2.5946298
0 3.1248589
0 3.379528
0 2.7820666
0 2.655951
0 2.7089748
0 3.1014159
0 3.198525
0 1.7074529
0 3.2679272
0 3.2683172
0 3.3533883
0 2.9607377
0 3.293312
0 3.2389522
0 2.5585587
0 2.5175478
0 3.3074017
0 3.2630682
0 3.128894
0 3.3475566
0 2.3642647
0 2.5757217
0 3.0583787
0 2.9741259
0 3.3716938
0 3.2409177
0 2.685136
0 3.007237
0 2.671015
0 3.3488293
0 3.1397057
0 3.3318853
0 2.9810426
0 3.357915
0 3.0405266
0 2.3656175
0 3.3140283
0 3.1621156
0 3.3891366
0 2.6070545
0 2.5834014
0 3.3952217
0 3.0177052
0 2.9784029
0 3.149425
0 3.3898404
0 2.3214836
0 3.0191364
0 2.9081302
0 2.7047448
0 2.862861
0 2.7506344
0 2.8978577
0 3.3208642
0 3.0502326
0 3.0253043
0 2.9343698
0 3.0164845
0 2.937532
0 3.0463297
0 3.0817788
0 2.5127962
0 2.668437
0 3.373491
0 3.3354797
0 2.925143
0 2.8632147
0 2.3463206
0 3.0679665
0 2.8677073
0 2.701715
0 3.354685
0 2.6469703
0 3.30656
0 3.3366773
0 3.331195
0 3.0289176
0 2.6964383
0 3.1540484
0 3.008501
0 2.8660138
0 2.9853325
0 3.2479014
0 2.8840854
0 3.1485858
0 3.267418
0 2.6548507
0 2.628023
0 3.171713
0 3.2063172
0 2.2206848
0 2.2321181
0 3.257687
0 3.0956273
0 2.4716256
0 3.304806
0 3.0884914
0 2.714437
0 3.3823645
0 3.0469184
0 3.062076
0 3.308212
0 3.2444377
0 2.5612404
0 3.1505945
0 3.3900077
0 2.2316978
0 3.3494499
0 2.9659696
0 3.1918557
0 3.3326552
0 2.4878118
0 2.6198123
0 2.3626232
0 3.2649837
0 2.3556542
0 3.0903733
0 2.8232818
0 1.6129184
0 2.419845
0 3.1481748
0 3.3479357
0 2.831876
0 2.794137
0 2.6503935
0 2.485973
0 3.2631671
0 2.1453297
0 3.359449
0 2.838843
0 2.745809
0 2.6753502
0 2.5974574
0 2.2764559
0 2.566519
0 3.3819375
0 2.9803996
0 2.8653069
0 2.8401332
0 2.7739453
0 3.346582
0 2.987988
0 1.8361117
0 3.1503437
0 3.125034
};
\addplot [darkorange25512714]
table {%
-0.075 4.383432
0.075 4.383432
};


%%PROCESSED BUT NOT PROTECTED

\addplot [black]
table {%
0.425 3.87224325
0.575 3.87224325
0.575 4.34285615
0.425 4.34285615
0.425 3.87224325
};
\addplot [black]
table {%
0.5 3.87224325
0.5 3.1668653
};
\addplot [black]
table {%
0.5 4.34285615
0.5 4.8728657
};
\addplot [black]
table {%
0.4625 3.1668653
0.5375 3.1668653
};
\addplot [black]
table {%
0.4625 4.8728657
0.5375 4.8728657
};
\addplot [black, mark=o, mark size=0.3, mark options={solid,fill opacity=0}, only marks]
table {%
0.5 3.025674
0.5 2.480098
0.5 2.2368307
0.5 3.1558447
0.5 3.1012943
0.5 2.8751972
0.5 2.7962618
0.5 3.1642203
0.5 3.0326815
0.5 2.9017496
0.5 2.6908722
0.5 3.1595507
0.5 2.7108545
0.5 3.0189245
0.5 2.7187152
0.5 3.1184196
0.5 3.0041885
0.5 3.0453458
0.5 3.0642498
0.5 2.6555781
0.5 3.0615215
0.5 3.1636927
0.5 2.5213041
0.5 2.9319937
0.5 2.5264804
0.5 2.812016
0.5 2.4807575
0.5 3.0297773
0.5 2.7876823
0.5 3.1581542
0.5 3.1420224
0.5 2.2499862
0.5 2.3471954
0.5 2.9026704
0.5 3.1388686
0.5 2.0479505
0.5 2.9503107
0.5 2.6812227
0.5 2.9358144
0.5 2.9110868
0.5 2.4175274
0.5 3.0871978
0.5 3.061021
0.5 2.8814473
0.5 2.7837234
0.5 2.6326127
0.5 2.9131248
0.5 2.878755
0.5 3.1429145
0.5 2.9953692
0.5 3.1196225
0.5 2.4525607
0.5 2.3139873
0.5 2.6086707
0.5 3.144391
0.5 2.7299023
0.5 2.9273267
0.5 2.375062
0.5 3.0222208
0.5 2.1191683
0.5 3.1477237
0.5 2.7502263
0.5 2.7625964
0.5 2.9615781
0.5 2.678743
0.5 3.1492195
0.5 3.0421107
0.5 2.9726717
0.5 3.0782092
0.5 2.3160973
0.5 2.9982698
0.5 2.3228996
0.5 2.2518806
0.5 2.4286447
0.5 3.1153889
0.5 2.9598002
0.5 2.9036798
0.5 2.4321532
0.5 2.6348548
0.5 3.0968802
0.5 3.0449307
0.5 2.4966674
0.5 2.8979044
0.5 3.0139604
0.5 2.942171
0.5 3.057849
0.5 2.4999533
0.5 3.087058
0.5 2.5218794
0.5 2.9541636
0.5 3.1190875
0.5 2.453314
0.5 2.9192004
0.5 2.6840193
0.5 2.6379232
0.5 2.5554311
0.5 2.598836
0.5 3.1247897
0.5 2.8101652
0.5 3.164066
0.5 2.9701002
0.5 2.9778018
0.5 2.7948709
0.5 3.0491712
0.5 2.6107929
0.5 2.9923859
0.5 2.3422253
0.5 2.680241
0.5 2.6131856
0.5 2.9535973
0.5 3.0261364
0.5 2.95748
0.5 3.1445482
0.5 2.5323768
0.5 3.0351865
0.5 2.4779692
0.5 2.8999639
0.5 2.8411233
0.5 3.1018736
0.5 2.8312573
0.5 2.7160487
0.5 2.6292753
0.5 2.3280432
0.5 1.8284874
0.5 2.521915
0.5 2.777356
0.5 2.200347
0.5 2.7515018
0.5 2.3014274
0.5 2.540702
0.5 3.0784192
0.5 2.6494021
0.5 3.0615213
0.5 3.0144322
0.5 2.8697321
0.5 2.954957
0.5 3.110782
0.5 3.1592805
0.5 2.6631465
0.5 2.5826652
0.5 2.4952264
0.5 1.9316075
0.5 3.0843818
0.5 2.8265204
0.5 2.5854983
0.5 2.6417313
0.5 3.0798552
0.5 3.0172598
0.5 2.328397
0.5 2.8611326
0.5 2.9399915
0.5 2.6813607
0.5 2.9716175
0.5 2.3767955
0.5 2.5290127
0.5 3.1158357
0.5 1.8221109
0.5 2.6577904
0.5 2.6124516
0.5 2.6300566
0.5 2.9487078
0.5 2.664202
0.5 2.838954
0.5 2.1057312
0.5 2.711392
0.5 2.891586
0.5 3.132168
0.5 3.1500983
0.5 2.8473837
0.5 2.9682093
0.5 3.113773
0.5 2.6640737
0.5 3.1107826
0.5 2.3938503
0.5 3.1521869
};
\addplot [darkorange25512714]
table {%
0.425 4.1384335
0.575 4.1384335
};


%%PROTECTED WITH PROPOSED

\addplot [black]
table {%
0.925 3.8348333
1.075 3.8348333
1.075 4.3295164
0.925 4.3295164
0.925 3.8348333
};
\addplot [black]
table {%
1 3.8348333
1 3.0988808
};
\addplot [black]
table {%
1 4.3295164
1 4.8634195
};
\addplot [black]
table {%
0.9625 3.0988808
1.0375 3.0988808
};
\addplot [black]
table {%
0.9625 4.8634195
1.0375 4.8634195
};
\addplot [black, mark=o, mark size=0.3, mark options={solid,fill opacity=0}, only marks]
table {%
1 2.8539762
1 3.0755072
1 2.4080377
1 2.6279688
1 3.0600019
1 2.9064999
1 2.1140208
1 2.6745079
1 2.728594
1 2.824751
1 2.7697964
1 3.003463
1 2.6518683
1 2.6560886
1 2.8350236
1 2.8581612
1 3.0090523
1 2.9676807
1 2.6621828
1 2.6519217
1 3.0037887
1 2.8395336
1 2.8194911
1 3.0914805
1 2.331781
1 2.544593
1 2.8926582
1 2.2305605
1 2.1723502
1 2.1287436
1 2.9804447
1 2.8715413
1 3.0463288
1 3.0630002
1 2.8089728
1 2.6876998
1 2.9010541
1 2.887492
1 2.9082274
1 2.9468927
1 2.630076
1 3.0199847
1 2.997558
1 2.7881334
1 3.0719523
1 2.996131
1 1.9476016
1 2.8632169
1 2.4699976
1 2.9352102
1 2.6824512
1 2.2351534
1 3.0051088
1 2.9555535
1 2.972893
1 2.4475086
1 3.0559194
1 2.5486376
1 3.0598102
1 2.8332882
1 2.9906032
1 2.9572692
1 2.6878316
1 2.8034282
1 2.6497233
1 3.0686834
1 3.051936
1 2.7957778
1 3.0573819
1 3.016989
1 2.9429252
1 2.7013328
1 3.0871027
1 1.9682488
1 3.0900004
1 2.6845014
1 2.7746665
1 3.0624
1 2.884039
1 2.8767085
1 2.553493
1 2.8561158
1 2.9387512
1 3.0704782
1 2.984923
1 3.0777283
1 3.0613723
1 2.9864464
1 2.5735297
1 3.0046928
1 3.0673354
1 2.8503149
1 2.63469
1 2.186009
1 3.0395186
1 2.2867875
1 3.035803
1 3.0507317
1 2.9537432
1 3.0361476
1 1.867933
1 3.0272536
1 2.7610357
1 2.8010478
1 2.4520159
1 3.0855885
1 3.0722742
1 3.0656312
1 2.0942652
1 1.6382468
1 2.3922834
1 2.199526
1 2.5541968
1 2.7572124
1 3.0582244
1 3.0163047
1 2.6185584
1 3.0770502
1 2.666617
1 2.4820058
1 2.904757
1 2.9641323
1 2.5280473
1 2.7742858
1 3.0729556
1 2.449059
1 3.0449142
1 2.9173448
1 2.98385
1 2.9668913
1 2.7991195
1 3.0706658
1 3.0715606
1 2.3320136
1 3.018931
1 2.9121857
1 3.0755482
1 3.0808284
1 3.0827098
1 2.7016985
1 2.879744
1 3.0845134
1 2.6176753
1 3.079268
};
\addplot [darkorange25512714]
table {%
0.925 4.114546
1.075 4.114546
};

%%GLOBAL

\addplot [black]
table {%
1.425 3.9860984
1.575 3.9860984
1.575 4.46313795
1.425 4.46313795
1.425 3.9860984
};
\addplot [black]
table {%
1.5 3.9860984
1.5 3.2757275
};
\addplot [black]
table {%
1.5 4.46313795
1.5 5.037
};
\addplot [black]
table {%
1.4625 3.2757275
1.5375 3.2757275
};
\addplot [black]
table {%
1.4625 5.037
1.5375 5.037
};
\addplot [black, mark=o, mark size=0.3, mark options={solid,fill opacity=0}, only marks]
table {%
1.5 3.0284848
1.5 3.239885
1.5 3.1508281
1.5 3.1348727
1.5 2.7130303
1.5 2.8881636
1.5 3.0239542
1.5 2.2047043
1.5 1.8215915
1.5 2.864317
1.5 2.576278
1.5 3.0674524
1.5 2.9622421
1.5 2.922231
1.5 2.7010896
1.5 2.6721523
1.5 2.3652108
1.5 2.9308224
1.5 3.0842676
1.5 2.962154
1.5 2.9799798
1.5 2.4453971
1.5 3.221721
1.5 3.1277254
1.5 3.1523347
1.5 2.6293628
1.5 3.135048
1.5 2.7740889
1.5 2.6021357
1.5 3.064532
1.5 3.0501423
1.5 3.0950017
1.5 2.8706858
1.5 2.8533223
1.5 2.750358
1.5 2.866955
1.5 3.0336876
1.5 2.8977025
1.5 2.7046585
1.5 3.192762
1.5 3.237792
1.5 2.58343
1.5 2.3686123
1.5 3.2696812
1.5 2.7564912
1.5 2.9672184
1.5 2.9059327
1.5 2.8767815
1.5 3.1992974
1.5 2.2226496
1.5 3.258039
1.5 2.173933
1.5 3.0857096
1.5 2.4720583
1.5 2.937127
1.5 3.241477
1.5 2.5618937
1.5 3.207587
1.5 2.6555343
1.5 3.1607788
1.5 3.2462142
1.5 2.322101
1.5 3.15475
1.5 2.487885
1.5 2.7292976
1.5 3.0607698
1.5 1.711322
1.5 3.2425408
1.5 2.5174515
1.5 2.5469675
1.5 2.1452487
1.5 3.2142425
1.5 3.0475767
1.5 2.6852767
1.5 2.9797661
1.5 3.0083838
1.5 2.9771085
1.5 2.2151718
1.5 3.1509244
1.5 2.7975576
1.5 2.8382745
1.5 2.9871085
1.5 2.79471
1.5 2.3266275
1.5 2.928076
1.5 3.0902421
1.5 2.3750958
1.5 3.2290244
1.5 2.6158688
1.5 3.0281215
1.5 3.0251412
1.5 2.5950675
1.5 3.0744162
1.5 2.486437
1.5 2.7143483
1.5 3.2464025
1.5 1.9968537
1.5 3.2025466
1.5 2.7753296
1.5 2.7770915
1.5 1.8145583
1.5 2.5031087
1.5 3.0964215
1.5 1.7420249
1.5 3.0070796
1.5 3.068412
1.5 2.8631046
1.5 3.1918197
1.5 3.0622025
1.5 3.006326
1.5 2.9880261
1.5 2.39076
1.5 3.2409263
1.5 3.0100276
1.5 2.8243012
1.5 3.0968788
1.5 2.6182415
1.5 2.6212027
1.5 2.9760318
1.5 2.8680956
1.5 2.692297
1.5 2.6687677
1.5 2.6339095
1.5 3.0169578
1.5 2.9946232
1.5 2.2640874
1.5 2.7503552
1.5 3.229179
1.5 2.6907687
1.5 2.6723924
1.5 3.0053692
1.5 2.7039275
1.5 3.2669094
1.5 3.0883381
1.5 2.7900655
1.5 2.782237
1.5 2.5580277
1.5 2.2314456
1.5 2.5929515
1.5 2.6614678
1.5 2.7288826
1.5 2.7461092
1.5 2.165387
1.5 2.5587869
1.5 2.6156013
1.5 3.1618328
1.5 2.6030056
1.5 2.8311763
1.5 3.0257635
1.5 3.081462
1.5 2.8601255
1.5 3.1293132
1.5 3.2382095
1.5 3.2622309
1.5 2.6442652
1.5 3.188528
1.5 2.6610367
1.5 2.2299578
1.5 2.7033072
1.5 2.642878
1.5 3.0567615
1.5 2.3459353
1.5 1.9077789
1.5 2.2779036
1.5 2.6539314
1.5 2.9763389
1.5 2.5998464
1.5 2.212068
1.5 3.1522062
1.5 3.116949
1.5 2.9876254
1.5 3.1262474
1.5 2.0141885
1.5 2.2608545
1.5 3.1709766
1.5 2.6195543
1.5 2.5803723
1.5 2.5602999
1.5 2.615073
1.5 2.9085505
1.5 3.1965485
1.5 2.9661293
1.5 2.6741247
1.5 2.386773
1.5 2.5129554
1.5 2.9570794
1.5 3.079237
1.5 3.0446076
1.5 2.6687024
1.5 2.863574
1.5 2.2212417
1.5 3.1029065
1.5 2.7206109
1.5 3.0805118
1.5 2.3637934
1.5 3.1391466
1.5 2.419843
1.5 3.2564683
1.5 2.3755808
1.5 3.0875943
1.5 3.19949
1.5 3.2379775
1.5 2.6982303
1.5 2.6508555
1.5 2.9607244
1.5 2.5859284
1.5 2.6771708
1.5 3.2085896
1.5 2.9775956
1.5 3.2569704
1.5 1.9010719
1.5 3.1634653
1.5 2.4508822
1.5 2.755617
1.5 2.2793086
1.5 1.8498523
1.5 3.1368172
1.5 2.5458868
1.5 2.9967122
1.5 3.0413995
1.5 3.0188084
1.5 3.206171
1.5 1.9471954
1.5 2.02977
1.5 3.226004
1.5 3.1371837
1.5 3.2447193
1.5 2.4964051
1.5 2.9730701
1.5 3.2655473
1.5 2.832571
1.5 2.9737575
1.5 1.8367484
1.5 3.2034268
1.5 3.268858
1.5 3.2057812
1.5 3.2230403
1.5 3.0283928
1.5 2.429087
1.5 2.7507114
1.5 2.4346576
1.5 3.128517
1.5 3.2416615
1.5 2.5178227
1.5 3.2013738
1.5 3.143982
1.5 2.6219037
1.5 3.214593
1.5 2.3628774
1.5 2.7759094
1.5 2.872948
1.5 2.6356435
1.5 2.49823
1.5 3.23978
1.5 2.0913599
1.5 3.2401412
1.5 2.9336925
1.5 3.055401
1.5 2.8304422
1.5 1.611594
1.5 2.5667434
1.5 2.5089393
1.5 2.2883573
1.5 2.3542876
1.5 2.6887355
1.5 3.0500834
1.5 3.2605567
1.5 3.0437415
1.5 2.5998375
1.5 3.0246992
1.5 2.696213
1.5 3.1929548
1.5 3.1698513
1.5 2.667111
1.5 2.943146
1.5 3.1656256
1.5 2.46597
1.5 3.2671313
1.5 2.7016053
1.5 2.6851227
1.5 3.1515653
1.5 3.162715
1.5 2.7935221
1.5 2.6926186
1.5 3.2609158
1.5 2.785523
1.5 3.2524383
1.5 3.016426
1.5 2.8007407
1.5 3.1770618
1.5 2.9210248
1.5 3.2626922
1.5 2.9774883
1.5 3.1343148
1.5 2.5382655
1.5 3.1491632
1.5 3.1045518
1.5 3.1472542
1.5 2.681902
1.5 2.4378655
};
\addplot [darkorange25512714]
table {%
1.425 4.23745155
1.575 4.23745155
};


%%TDPSOLA

\addplot [black]
table {%
1.925 3.2351109
2.075 3.2351109
2.075 4.027795
1.925 4.027795
1.925 3.2351109
};
\addplot [black]
table {%
2 3.2351109
2 2.049495
};
\addplot [black]
table {%
2 4.027795
2 4.868727
};
\addplot [black]
table {%
1.9625 2.049495
2.0375 2.049495
};
\addplot [black]
table {%
1.9625 4.868727
2.0375 4.868727
};
\addplot [black, mark=o, mark size=0.3, mark options={solid,fill opacity=0}, only marks]
table {%
2 2.0256326
2 1.6578492
2 1.69306
2 2.0256221
2 1.959413
2 1.5848184
2 1.7830751
2 2.0276506
2 1.8378605
2 1.9316621
2 1.8120153
2 1.7157826
2 1.9075109
2 1.8079921
2 1.9120868
2 1.5570488
2 1.6045446
2 1.9717205
2 1.7369473
2 1.8181375
2 1.7345743
2 1.1321502
2 1.5165153
2 2.0107043
2 1.8536334
2 1.8928007
2 1.9596307
2 1.8334522
2 1.6914436
2 1.694243
2 1.1865088
2 1.6150614
2 1.7116188
2 1.5415981
2 1.5958598
2 1.2128106
2 1.9291736
2 1.9044629
2 1.7985947
2 1.6396992
2 1.6988983
2 1.8486043
2 1.8158867
2 2.0064056
2 1.8792735
2 1.9234807
2 1.7184018
2 2.0284734
2 1.4348599
2 1.8491807
2 1.9932564
2 1.9772806
2 1.8541715
2 1.8514556
2 1.5709233
2 1.4393651
2 1.86429
2 1.8327599
2 1.8323394
2 1.1426867
2 1.6422696
2 1.7117016
2 1.8090005
2 2.0051847
2 2.000313
2 1.8808479
2 1.8159448
2 1.9029362
2 1.2613204
2 1.6923372
2 1.2463237
2 1.8439854
2 1.0890832
2 2.0064623
2 2.0136335
2 1.9639378
2 1.9755518
2 1.7449722
2 2.013026
2 1.9198496
2 1.05201
2 1.5870289
2 2.0377092
2 1.3628637
2 1.9236468
2 1.733707
2 1.8228196
2 1.9086127
2 1.3223946
2 2.0217772
2 1.7647796
2 1.4322275
2 1.8075023
2 1.7501903
2 1.7865626
2 2.0235188
2 1.7363331
2 2.0089388
2 2.0204818
2 1.8906615
2 1.7222785
2 1.8122306
2 1.5505495
2 1.9598829
2 1.9827622
2 1.7652962
2 1.9332541
2 1.5609716
2 0.889323
2 2.0172985
2 1.8855023
2 1.4343364
2 1.7522674
2 1.955702
2 1.891446
2 1.8074538
2 1.7009177
2 1.8068244
2 1.9449108
2 2.0018537
2 1.7775309
2 1.3472344
2 1.6002578
2 1.5725749
2 1.9900318
2 1.4244252
2 1.1444514
2 1.2985644
2 1.51352
2 1.9030032
2 2.016569
2 1.9795965
};
\addplot [darkorange25512714]
table {%
1.925 3.6641643
2.075 3.6641643
};


\end{axis}


\end{tikzpicture}

==> figures/scores_histograms/calibrated_scores_histogram.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-5.5, xmax=5.5,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=1125.6,
ytick style={color=black},
height=3.5cm,
width=0.4\textwidth
]
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-1.34206271474174,0) rectangle (axis cs:-1.02964210560473,275);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-1.02964210560473,0) rectangle (axis cs:-0.717221496467719,132);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-0.717221496467719,0) rectangle (axis cs:-0.404800887330708,248);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-0.404800887330708,0) rectangle (axis cs:-0.0923802781936971,54);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-0.0923802781936971,0) rectangle (axis cs:0.220040330943314,333);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:0.220040330943314,0) rectangle (axis cs:0.532460940080325,16);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:0.532460940080325,0) rectangle (axis cs:0.844881549217336,43);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:0.844881549217336,0) rectangle (axis cs:1.15730215835435,0);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:1.15730215835435,0) rectangle (axis cs:1.46972276749136,0);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:1.46972276749136,0) rectangle (axis cs:1.78214337662837,1072);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-1.34206271521178,0) rectangle (axis cs:-1.02964210200896,776);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-1.02964210200896,0) rectangle (axis cs:-0.717221488806144,338);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-0.717221488806144,0) rectangle (axis cs:-0.404800875603328,403);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-0.404800875603328,0) rectangle (axis cs:-0.0923802624005126,60);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-0.0923802624005126,0) rectangle (axis cs:0.220040350802303,298);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:0.220040350802303,0) rectangle (axis cs:0.532460964005119,12);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:0.532460964005119,0) rectangle (axis cs:0.844881577207935,23);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:0.844881577207935,0) rectangle (axis cs:1.15730219041075,0);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:1.15730219041075,0) rectangle (axis cs:1.46972280361357,0);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:1.46972280361357,0) rectangle (axis cs:1.78214341681638,172);
\end{axis}

\end{tikzpicture}


==> figures/scores_histograms/calibrated_scores_histogram_gt.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-5.5, xmax=5.5,
xtick style={color=black},
y grid style={darkgray176},
ymin=0, ymax=2177.7,
ytick style={color=black},
height=3.5cm,
width=0.4\textwidth
]
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-5.33003611948282,0) rectangle (axis cs:-4.46658468320668,8);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-4.46658468320668,0) rectangle (axis cs:-3.60313324693053,2);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-3.60313324693053,0) rectangle (axis cs:-2.73968181065439,3);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-2.73968181065439,0) rectangle (axis cs:-1.87623037437824,19);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-1.87623037437824,0) rectangle (axis cs:-1.0127789381021,12);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-1.0127789381021,0) rectangle (axis cs:-0.149327501825957,10);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:-0.149327501825957,0) rectangle (axis cs:0.714123934450186,11);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:0.714123934450186,0) rectangle (axis cs:1.57757537072633,23);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:1.57757537072633,0) rectangle (axis cs:2.44102680700247,11);
\draw[draw=none,fill=red,fill opacity=0.4] (axis cs:2.44102680700247,0) rectangle (axis cs:3.30447824327862,2074);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-5.33003615027013,0) rectangle (axis cs:-4.46658470922313,1544);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-4.46658470922313,0) rectangle (axis cs:-3.60313326817612,102);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-3.60313326817612,0) rectangle (axis cs:-2.73968182712912,54);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-2.73968182712912,0) rectangle (axis cs:-1.87623038608212,236);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-1.87623038608212,0) rectangle (axis cs:-1.01277894503512,38);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-1.01277894503512,0) rectangle (axis cs:-0.149327503988119,21);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:-0.149327503988119,0) rectangle (axis cs:0.714123937058883,6);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:0.714123937058883,0) rectangle (axis cs:1.57757537810588,7);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:1.57757537810588,0) rectangle (axis cs:2.44102681915288,2);
\draw[draw=none,fill=blue,fill opacity=0.4] (axis cs:2.44102681915289,0) rectangle (axis cs:3.30447826019989,72);
\end{axis}

\end{tikzpicture}

